Joint Geometry and Attribute Upsampling of Point Clouds Using Frequency-Selective Models with Overlapped Support

With the increasing demand of capturing our environment in three-dimensions for AR/ VR applications and autonomous driving among others, the importance of high-resolution point clouds rises. As the capturing process is a complex task, point cloud upsampling is often desired. We propose Frequency-Selective Upsampling (FSU), an upsampling scheme that upsamples geometry and attribute information of point clouds jointly in a sequential manner with overlapped support areas. The point cloud is partitioned into blocks with overlapping support area first. Then, a continuous frequency model is generated that estimates the point cloud's surface locally. The model is sampled at new positions for upsampling. In a subsequent step, another frequency model is created that models the attribute signal. Here, knowledge from the geometry upsampling is exploited for a simplified projection of the points in two dimensions. The attribute model is evaluated for the upsampled geometry positions. In our extensive evaluation, we evaluate geometry and attribute upsampling independently and show joint results. The geometry results show best performances for our proposed FSU in terms of point-to-plane error and plane-to-plane angular similarity. Moreover, FSU outperforms other color upsampling schemes by 1.9 dB in terms of color PSNR. In addition, the visual appearance of the point clouds clearly increases with FSU.

==> figures/flowgraph_geo_up.tex <==
% Flow chart for geometry upsampling

% Define block styles

\definecolor{colorflow}{rgb}{0.00000,0.44700,0.74100}%
\makeatletter
\newif\iftikz@ortho@preflush
\tikz@ortho@preflushtrue
\let\tikz@origtotarget\pgfutil@empty
\tikzset{
	|-/.style={to path={|- (\tikztotarget) \tikztonodes}},
	-|/.style={to path={-| (\tikztotarget) \tikztonodes}},
	*|/.style={to path={%
			\pgfextra
			\iftikz@shapeborder
			\tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
			\ifdim\pgf@y>\tikz@lasty\relax
			\edef\tikztostart{\tikztostart.north}%
			\else
			\edef\tikztostart{\tikztostart.south}%
			\fi
			\fi
			\endpgfextra
			(\tikztostart-|\tikztotarget) -- (\tikztotarget) \tikztonodes
	}},
	*-/.style={to path={%
			\pgfextra
			\iftikz@shapeborder
			\tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
			\ifdim\pgf@x>\tikz@lastx\relax
			\edef\tikztostart{\tikztostart.east}%
			\else
			\edef\tikztostart{\tikztostart.west}%
			\fi
			\fi
			\endpgfextra
			(\tikztostart|-\tikztotarget) -- (\tikztotarget) \tikztonodes
	}},
	|*/.style={to path={%
			\pgfextra
			\tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
			\iftikz@shapeborder
			\let\tikz@origtotarget\tikztotarget
			\ifdim\pgf@y>\tikz@lasty\relax
			\edef\tikztotarget{\tikztotarget.south}%
			\else
			\edef\tikztotarget{\tikztotarget.north}%
			\fi
			\fi
			\endpgfextra
			(\tikztostart) -- (\tikztostart|-\tikztotarget) \tikztonodes \ifx\tikz@origtotarget\pgfutil@empty\else\iftikz@ortho@preflush(\tikz@origtotarget)\fi\fi
	}},
	-*/.style={to path={%
			\pgfextra
			\tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
			\iftikz@shapeborder
			\let\tikz@origtotarget\tikztotarget
			\ifdim\pgf@x>\tikz@lastx\relax
			\edef\tikztotarget{\tikztotarget.west}%
			\else
			\edef\tikztotarget{\tikztotarget.east}%
			\fi
			\fi
			\endpgfextra
			(\tikztostart) -- (\tikztostart-|\tikztotarget) \tikztonodes \ifx\tikz@origtotarget\pgfutil@empty\else\iftikz@ortho@preflush(\tikz@origtotarget)\fi\fi
	}},
	node as new start/.is if=tikz@ortho@preflush
}


\tikzset{%
	back group/.style={fill=yellow!20,rounded corners, draw=black!50, dashed, inner xsep=12pt, inner ysep=11pt, yshift=-5pt}
}

\tikzstyle{decision} = [diamond, draw, fill=white!15, 
text width=4.5em, text badly centered, node distance=3cm, inner sep=0pt]
\tikzstyle{block} = [rectangle, draw, fill=white!15, 
text width = 20em, text centered, rounded corners, minimum height=2em] % Standard Block
\tikzstyle{block2} = [rectangle, draw=colorflow, fill=white!15, line width = 2pt,
text width = 20em, text centered, rounded corners, minimum height=2em] % Standard Block blaue Umrandung für 2D
\tikzstyle{blockk} = [rectangle, draw, fill=colorflow, 
text width = 20em, text centered, rounded corners, minimum height=2em] % Block
\tikzstyle{block3} = [rectangle, draw, fill=white!15, 
text width = 10em, text centered, rounded corners, minimum width=10em, minimum height=2em] % Schmaler Block links
\tikzstyle{block4} = [rectangle, draw, fill=white!15, 
text width = 6em, text centered, rounded corners, minimum width=6em, minimum height=2em] % Schmaler Block rechts
\tikzstyle{blockk} = [rectangle, draw, fill=colorflow, 
text width = 20em, text centered, rounded corners, minimum height=2em] % Block
\tikzstyle{blockkk} = [rectangle, draw=white, fill=white!15, 
text width = 20em, text centered, rounded corners, minimum height=2em] % Block ohne Rahmen
\tikzstyle{blocksummarize} = [rectangle, draw, fill=white!15, line style=dashed,
text width = 20em, text centered, rounded corners, minimum height=2em] % Block zum Zusammenfassen anderer Blöcke
\tikzstyle{line} = [draw, -latex']
\tikzstyle{cloud} = [draw, ellipse,fill=white!20, node distance=5cm,
minimum height=2em]

\makeatother
\begin{tikzpicture}[node distance = 1.5cm, auto]
	% Place nodes
	\node [blockkk] (init) {Low-resolution point cloud};
	\node[block, below=of init] (blockpartitioning) {Block partitioning with support area};
	\node [block, below of=blockpartitioning, node distance = 1.2cm] (var) {Determining variances};
	\node [block, below of=var] (smallvar) {Select smallest variance to be modelled};
	%    \node [block, below of=graph] (minspan) {Create minimum spanning tree $\mathcal{M} \subset \mathcal{G}$};
	%    \node [block, below of=smallvar] (deltatilde) {Calculate $\Delta\widetilde{x}_{ij}$ and $\Delta\widetilde{y}_{ij}$};
	%    \node [block, below of=deltatilde] (tilde) {Calculate $\widetilde{x}_{j}$ and $\widetilde{y}_{j}$};
	
	\node [block3, below of=smallvar, left of= smallvar, node distance = 1.95cm] (residual) {Calculate residual $r^{(\nu)}[x',y']$};
	\node [block3, below of=residual] (energy) {Calculate residual energy decrease $\Delta E^{(\nu)}$ for every basis function};
	\node [block3, below of = energy] (selection) {Selection of best fitting basis function};
	\node [decision, below of=selection, node distance = 2.5cm] (stop) {Stopping criterium met?};
	\node [block4, below of = smallvar, right of=smallvar, right = .5em of residual] (2dims) {Estimate points in \(x'-y'\)-plane using triangulation};
	\node [block, below of= stop, right of = stop, node distance = 2.5cm] (mesh) {Obtain \(\hat{z}'\) of additional points.};
	\node [decision, below of = 2dims] (enoughpoints) {Enough points generated?};
	%    \node [block, below of=mesh, node distance = 1.6cm] (3to2) {Assign reconstructed values to $\{x, y, z\}\in \mathbb{R}^3$};
	\node [blockkk, below of=mesh, node distance = 1cm] (finish) {High-resolution point cloud};
	
	% Create coordinates
	\coordinate[right of=residual] (a1);  %This is so the path doesn't intersect the diagram 
	\coordinate[right of=stop] (e1); 
	\coordinate[right of=enoughpoints] (e2);
	\coordinate[left of=stop](helper);
	
	% Draw edges
	\path [line] (init) -- (blockpartitioning);
	\path [line] (blockpartitioning) -- (var);
	\path [line] (var) -- (smallvar);
	%    \path [line] (graph) -- (minspan);
	%    \path [line] (smallvar.-170) -- (residual);
	\path [line] (smallvar) to[*|]  (residual);
	\path [line] (residual)  -- (energy);
	\path [line] (energy) -- (selection);
	\path [line] (selection) -- (stop);
	\path [line] (stop) -| node [near start]{No}([xshift=1.2cm]e1) -- node[sloped, anchor=center, above, text width = 5cm](atest){Generated model $g^{(\nu)}[x',y']$}([xshift=1.2cm]a1) -- (residual);
	%    \path [line] (stop.south) -- node[near start]{Yes} (mesh.171.8);
	\path [line] (stop) to[|*] node[near start]{Yes} (mesh);
	\path [line] (mesh) -- (finish);
	%    \path [line] (3to2) -- (finish);
	%    \path [line] (smallvar.-7.8) -- (2dims);
	\path [line] (smallvar) to[*|]  (2dims);
	\path [line] (2dims) -- (enoughpoints);
	\path [line] (enoughpoints) to[|*] node[near start](yesenough){Yes} (mesh);
	\path [line] (enoughpoints.east) -| node [near start](notenough){No}([xshift=.5cm]e2) |-  (2dims.east);
	
	\path (atest) +(0.3, 10) coordinate (a2);
	
	\begin{scope}[on background layer]
		%    		\node (bk1) [back group] [fit=(var) (a2) (tilde)] {};
		\node (bk2) [back group] [fit=(residual) (atest) (stop)] {};
		%    		\node[anchor=south east,inner sep=1pt,outer sep=1pt,opacity=0.5,font=\sffamily\bfseries,text=gray] at (bk1.south east){3D to 2D transform};
		\node[anchor=south east,inner sep=1pt,outer sep=1pt,opacity=0.5,font=\sffamily\bfseries,text=gray] at (bk2.south east){}; %{FSGU - Sec. \ref{Sec:FSGU}};%FSGU - Sec. \ref{Sec:FSGU}};
	
	% Scope for right path and sec. 2.2
	%    		\node (bk3) [back group] [fit=(2dims)(notenough)(yesenough) (enoughpoints)] {};
	%    		\node[anchor=south east,inner sep=1pt,outer sep=1pt,opacity=0.5,font=\sffamily\bfseries,text=gray] at (bk3.south east){Point Locs. - Sec. \ref{sec:pointlocs}};%FSGU - Sec. \ref{Sec:FSGU}};
\end{scope}

%    % Scope for right path and sec. 2.2
%        \begin{scope}[on background layer]
%    		\node (bk3) [back group] [fit=(2dims) (enoughpoints)] {};
%    		\node[anchor=south east,inner sep=1pt,outer sep=1pt,opacity=0.5,font=\sffamily\bfseries,text=gray] at (bk3.south east){};%FSGU - Sec. \ref{Sec:FSGU}};
%    \end{scope}

%    \draw [dashed, ->] (Val.south) -- (Val|-Interp.north);
%\draw [dashed, ->] (Val.south|-Interp.south) -- (Val|-int1.north);
%\draw [dashed, ->] (Val.south|-int1.south) -- (Val|-res1.north);
%\draw [dashed, ->] (Val.south|-res1.south) -- (Val|-int2.north);
%\draw [dashed, ->] (Val.south|-int2.south) -- (Val|-Train_net.north);

\end{tikzpicture}



%\tikzstyle{block} = [rectangle, rounded corners, minimum width=.4\columnwidth, minimum height=1cm, text width=3.5cm, text centered, draw=black] % standard block\\
%\tikzstyle{block_wide} = [rectangle, rounded corners, minimum width=\columnwidth, minimum height=1cm, text width=3.5cm, text centered, draw=black] % wide block
%\tikzstyle{hide} = [rectangle, minimum width=\columnwidth, minimum height=1cm, text width=\columnwidth, text centered]
%\tikzstyle{arrow} = [thick,->,>=stealth]
%
%\begin{tikzpicture}%[node distance = 1.5cm, auto]
%		% Draw nodes
%		% Combined upper part
%	\node[hide] (lowres) {Low-resolution input point cloud};
%	\node[block_wide, below=of lowres] (blockpartitioning) {Block partitioning};
%	\node [block_wide, below=of blockpartitioning, node distance = 1.2cm] (var) {Determining variances};
%	\node [block_wide, below=of var] (smallvar) {Select smallest variance to be modelled};
%	
%	% Left part
%	\node[block, below=of smallvar.south west, anchor=north west] (residual) {Calculate residual};
%	\node[block, below=of residual] (residualenergy) {Calculate residual energy decrease};
%	\node[block, below=of residualenergy] (bf_selection) {Select best fitting basis function};
%	\node[block, below=of bf_selection] (stop) {Stopping criterium met?};
%	
%	% Right part
%	\node[block,  below=of smallvar.south east, anchor=north east] (triangulate) {Triangulate \(x'\) and \(y'\)};
%	\node[block, below=of triangulate] (add) {Add $\hat{x}$ and $\hat{y}$ on half of triangulated edges};
%	\node[block, below=of add] (enough) {Enough points generated?};
%	
%	% Combined lower part
%	\node[hide, below=of stop, centered] (highres) {High-resolution output point cloud};
%	
%	% Draw arrows
%%	\draw[arrow] (lowres) -- (geo);
%%	\draw[arrow] (geo.east) -- (att.west);
%%	\draw[arrow] (att) -- (highres);
%\end{tikzpicture}
